Alpha-Fair Routing in Urban Air Mobility with Risk-Aware Constraints

In the vision of urban air mobility, air transport systems serve the demands of urban communities by routing flight traffic in networks formed by vertiports and flight corridors. We develop a routing algorithm to ensure that the air traffic flow fairly serves the demand of multiple communities subject to stochastic network capacity constraints. This algorithm guarantees that the flight traffic volume allocated to different communities satisfies the \emph{alpha-fairness conditions}, a commonly used family of fairness conditions in resource allocation. It further ensures robust satisfaction of stochastic network capacity constraints by bounding the coherent risk measures of capacity violation. We prove that implementing the proposed algorithm is equivalent to solving a convex optimization problem. We demonstrate the proposed algorithm using a case study based on the city of Austin. Compared with one that maximizes the total served demands, the proposed algorithm promotes even distributions of served demands for different communities.

==> figs/alpha.tex <==
\begin{figure}
    \centering
\begin{tikzpicture}
\begin{axis}[xmin=0, xmax=4, ymin=-10, ymax=3, samples=100, width=0.6\columnwidth,
height=0.3\columnwidth,
      scale only axis,
      legend pos=south east,
      label style={font=\footnotesize},
            tick label style={font=\footnotesize},
            legend style={font=\footnotesize}]
  \addplot[teal, thick, domain=0.01:4] {ln(x)};
  
  \addplot[blue, thick, domain=0.01:4] {-1/x};

  \addplot[red, thick, domain=0.6:4] {-1/(15*x^(15))};
  \legend{$\alpha=1$,$\alpha=2$,$\alpha=16$}
\end{axis}
\end{tikzpicture}
    \caption{\(\alpha\)-utility functions}
    \label{fig: alpha}
\end{figure}

==> related/related.tex <==
\section{Related Work}

==> routing/sarah.tex <==
\begin{comment}

\tc{blue}{Hey Yoyo. I think how I interpreted the risk measures may be slightly different. Just read the following and let me know what you think. For reference I'm using Shapiro's text on stochastic programming~\cite{shapiro2021lectures}.}

\tc{blue}{We model the network's link and node capacity vectors as a random variable $Z$, and assume that the union of capacity vectors under all possible operation conditions is a finite set. 
\begin{assumption}
    The node and link capacities are random variables $C$ and $D$ over a finite sample space $\Omega$---i.e., $|\Omega| < \infty$, $|\Omega| = N$.
\end{assumption} 
Under normal operating conditions, each outcome $c_i, d_i$ has probability $p_i$ of occurring. We denote this as the nominal probability distribution $p$. 
}


\tc{blue}{
Weather disturbances and emergency shutdowns causes $p$ the probability mass function to change. We model the change in the pmf as a new random variable $Z'$, which is defined over the same outcome space $\Omega$ as $Z$. We define the space of all random variables  over $\Omega$ with measurable pmf as $\mathcal{Z}$. Given flow vector $y$, we define a coherent risk measure $\rho_{\delta}(Z; y):\mathcal{Z} \mapsto \mathbb{R} \cup \{\pm \infty\}$ to evaluate the risk of violating constraint~\eqref{eqn: nl cap constraint}--- for a vehicle flow $y$ and risk threshold $\delta > 0$, $\rho_{\delta}(Z'; y)$ evaluates the risk of violating constraint~\eqref{eqn: nl cap constraint} under random variable $Z'$. For example, CVar evaluates the conditional expectation of the constraint function~\eqref{eqn: nl cap constraint} in the upper $\delta$ percentile. 
}

\tc{blue}{In particular, we assume that this risk measure is coherent~\cite[Sec.6.3]{shapiro2021lectures}---i.e. that it is convex, monotonic, translationally equivalent, and positively homogenous in random variable ${Z}$.   From the dual representation theorem, $\rho_{\delta}(Z; y)$ can be evaluated as~\eqref{eqn: crm}, where $\mathbb{Q}(\delta)$ is a convex set~\cite[Thm6.8]{shapiro2021lectures} for all values of $\delta$.(I think this better motivates Assumption 2). Instead of evaluating the constraint function ~\eqref{eqn: nl cap constraint} at the $\delta$ quantile under random variable $Z$, the dual representation theorem  allows $\rho_\delta(Z; y)$ to be computed as the supremum of~\eqref{eqn: nl cap constraint} over a set of pmfs, where the size of the set is controlled by $\delta$. This can be easier than finding the $\delta$ quantile of $Z$, which is like computing the cumulative distribution function of $Z$. }

\tc{blue}{To be risk-aware, we replace the constraint~\eqref{eqn: nl cap constraint} with the following bound on the coherent risk measure~\eqref{eqn: risk constraint} and evaluate measure deterministically via its dual form. The dual forms are given in the Appendix(I'm looking at the dual forms in the appendix, and I'm wondering maybe it's worth showing how you got the $g_{\delta}(q)$ for CVar and EVar?).}

    
\end{comment}
